CROSSLINE: Breaking "Security-by-Crash" based Memory Isolation in AMD SEV

AMD's Secure Encrypted Virtualization (SEV) is an emerging security feature on AMD processors that allows virtual machines to run on encrypted memory and perform confidential computing even with an untrusted hypervisor. This paper first demystifies SEV's improper use of address space identifier (ASID) for controlling accesses of a VM to encrypted memory pages, cache lines, and TLB entries. We then present the CROSSLINE attacks, a novel class of attacks against SEV that allow the adversary to launch an attacker VM and change its ASID to that of the victim VM to impersonate the victim. We present two variants of CROSSLINE attacks: CROSSLINE V1 decrypts victim's page tables or memory blocks following the format of a page table entry; CROSSLINE V2 constructs encryption and decryption oracles by executing instructions of the victim VM. We have successfully performed CROSSLINE attacks on SEV and SEV-ES processors.

==> 91-app1.tex <==
\section{Appendix: Extended Discussion}
\label{sec:appendix}

\subsection{Relation to Speculative Execution Attacks}

\atkname is \textit{not} a speculative execution attack. Meltdown~\cite{lipp:2018:meltdown}, Spectre~\cite{kocher:2019:spectre}, L1TF~\cite{van:2018:foreshadow}, and MDS~\cite{van:2019:ridl,schwarz:2019:zombieload,canella:2019:fallout} are prominent speculative execution attacks that exploit transiently executed instructions to extract secret memory data through side channels. In these attacks, instructions are speculatively executed while the processor awaits resolution of branch targets, detection of exceptions, disambiguation of load/store addresses, \etc. However, in the settings of \atknameOne, no instructions are executed, as the exceptions take place as soon as the frontend starts to fetch instructions from the memory. The other two variants of \atkname executes instructions with architecture-visible effects.

\atkname does not rely on micro-architectural side channels, either. Speculative execution attacks leverage micro-architectural side channels (\eg, cache side channels) to leak secret information to the program controlled by the attacker. In contrast, \atkname reveals data from the victim VM as page frame numbers, which can be learned by the hypervisor directly during page fault handling. 




==> 99-app-ndss.tex <==
\newpage
\newpage
\section*{Previous Reviews (NDSS 2021)}

%\textbf{We have attached the verbatim reviews from NDSS 2021 below and interleaved with our response to the comments. }

\subsection*{\textcolor{Maroon}{Review A}}
\bheading{Overall recommendation:}
3. Major revision

\bheading{Writing quality:}
4. Well-written

\bheading{Reviewer Confidence:}
3. Sufficient confidence

\bheading{Paper summary:}

The paper describes two attacks on AMD Secure Encrypted Virtualization (SEV). In both attacks, an attacker manipulates fields in the unprotected VMCB. The first attack can read page tables or other data that look like page table entries. The second attack version allows the attacker to arbitrarily read and write in the victim VM. The second attack does not work under SEV-SE and neither attack works under SEV-SNP.

\bheading{Strengths:}

+ The attacks are complex and interesting.

+ The attacks are relatively stealthy.

+ The paper is mostly well written.

\bheading{Weaknesses:}

- The work is somewhat incremental. The limitations of basic SEV are well known and a number of attacks with similar results have been published already.

- The impact of the attacks is limited. Version 2 does not work against SEV-SE, and neither version works against SEV-SNP.

\rebut{ As mentioned in the reviews, Google’s confidential VM already leverages SEV-ES for commercial services. We believe any violation of the SEV-protected VM’s confidentiality should be considered a real-world threat to users of the confidential cloud services, who typically have high-security demands. Even if the leakage is constrained to page tables, it already allows the attacker to learn the virtual address mapping inside the guest VM, breaking both KASLR and ASLR of applications. If this is not a real threat, the same argument can go against many other security papers aiming to break (K)ASLR.
In addition, any data and code blocks conformant to PTE formats can also be leaked. We have no doubt that these security-sensitive cloud customers would care about the attack. 
}

\bheading{Detailed comments for authors:}

I have read the paper with interest. The attacks are interesting and non-trivial. Overall, the paper seems well written.

This paper might have been an easy accept two years ago. However, at this time, two developments detract from the paper's message.

First, the (well known) limitations of basic SEV have been and are being fixed by AMD. With SEV-SE deployment inexorably rising and SEV-SNP on the not-too-distant horizon, basic SEV is becoming increasingly obsolete (at least from a security research perspective). This makes attacks on it less interesting.

Second, a number of similar attacks with similar results on basic SEV have been published over the past years. This attack uses a somewhat different strategy, and it is a little more stealthy, but there is no real surprise here. SEV leaves the VMCB unprotected.

A variant of version 1 also works against SEV-SE. This is significant. However, the paper does not make the case that this attack has a severe impact. Clearly, the adversary should not be able to read the victim's page tables, but what if he does? Being able to demonstrate a concrete negative impact of v1 on SEV-SE would strengthen the paper.

Stealth: What is the exact criterion for getting the "Stealthiness" checkmark in Table II? CROSSLINE is not undetectable in an absolute sense. The OS could try to monitor CR2, and there is a timing impact which may be observable.

\rebut{In SEV mode, Crossline V1 and V2 only change CR2 in the attacker VM’s VMCB, which makes Crossline attack completely stealthy. 
In SEV-ES mode, Crossline attack only affects the CR2 field in VMSA. The guest OS is hard to detect Crossline attack for two reasons: (1) The AE NPFs are transparent to the guest OS, which are directly trapped into the hypervisor, such that the guest OS does not have a chance to record the original value of CR2 to compare with. (2) Similarly, it is impossible to measure the slowdown of a single VMEXIT, since the AE NPFs are not trapped by the guest OS. The guest OS may observe a slowdown of its overall execution, if it has access to a trusted clock (which unfortunately we are not aware of on SEV), which is hard to be differentiated from running the VM on a crowded machine.
We’d like to open source our attack code and invite fellow researchers to build detection systems for CrossLine and similar attacks. 
}

What does "demystify" mean in Section III? Does the section contain information that is not provided in the processor manual or other obvious sources? If so, how was that information obtained.

\rebut{First, there is no existing document/article explaining the roles of ASID in SEV. This paper provides the first systematic summarization of how ASIDs are used for isolating VMs in SEV.
Second, some of the results come from empirical evaluation. For instance: (1) An SEV VM and a non-SEV VM with the same ASID can exist at the same time. However, their cache lines and TLB entries are isolated by additional tags. (2) The runtime restriction of ASID assignment is not documented in the whitepaper, so we had to run experiments to explore how the hypervisor could alter the ASID of a guest VM in a variety of settings. (3) We validated that the processor trusts the values inside VMCB without sufficient checks. We have made these clear in this revision.
}

\subsection*{\textcolor{Maroon}{Review B}}
\bheading{Overall recommendation:}
4. Minor revision

\bheading{Writing quality:}
4. Well-written

\bheading{Reviewer Confidence:}
3. Sufficient confidence

\bheading{Paper summary:}

This paper presents two attacks against AMD SEV and AMD SEV-ES called Crossline v1 and v2, which do not exploit the well-known lack of memory integrity protection in these versions of AMD SEV. Common to enabling both attacks is the hypervisor's ability to modify the ASID (address space ID) of an existing VM to collide with that of a target SEV or SEV-ES VM. With a modified ASID, the CPU decrypts memory contents with the memory encryption key of the victim VM, and using attacker-controlled nested page tables. AMD specifications state that this will "very likely" cause a fault. However, "very likely" is not "always". The Crossline v1 attack is able to read out the (SEV or SEV-ES) victim VM's complete page tables, and then also read out memory contents that comply with the constraints of legitimate page table entries. Crossline v2 against plain SEV can additionally execute a few instructions within the victim VM, which if carefully chosen allow complete violation of confidentiality and integrity.

\bheading{Strengths:}

+ Clear presentation of a subtle attack. Pretty clever technique, though the "highly likely" is a bit of a red flag in the SEV description.

+ Working implementations with good performance and stability.

+ Stealthy.

\bheading{Weaknesses:}

- AMD SEV and SEV-ES are already known to be vulnerable to a malicious hypervisor, so the real-world security impact is primarily confined to some additional analysis that should be performed against upcoming AMD SEV-SNP to ensure that it fully mitigates these attacks. However, if this does lead to changes in SNP, then it was quite worthwhile.

\rebut{Crossline is the only known stealthy attack that cannot be easily detected by guest VMs, which is ideal for a curious cloud service provider to perform non-intrusion attacks. There are no I/O interactions with the victim or negative impacts on its execution correctness.
In addition, it is not a justifiable reason to dismiss CrossLine simply based on its consequences---it exploits a different hardware design flaw and requires new attack techniques.
}

\bheading{Detailed comments for authors:}

This is a fairly clever attack technique and shows yet again why it is unwise to assume that something that is "highly likely" to decrypt to garbage (and cause a crash), doesn't always.

The paper talks about disclosure and discussion with AMD, but isn't entirely clear if AMD has been able to devise any mitigations. Are there any? Is there a CVE for this issue?

\rebut{We have reported several vulnerable hardware designs to AMD including: 1. The lack of ASID authentication and inappropriate “security-by-crash” principle. 2. The lack of triple fault reporting, which allows SEV and SEV-ES VM to resume from a triple fault by rewinding VMCB. 3. The VMSA check is only tied to VMSA’s physical address but not VMCB’s physical address, which makes Crossline work in SEV-ES. These vulnerabilities have been acknowledged by AMD. 
AMD does not plan to fix these vulnerabilities in SEV/SEV-ES, as they require some fundamental changes in the SEV design. Instead, as the attacks do not work on SEV-SNP, AMD plans to rely on SEV-SNP as a line of defense. But AMD engineers admit plans to move away from the “security-by-crash” principle in the future.
As the work has been acknowledged by AMD already, we felt less incentivized to file an CVE with Mitre. 
}

p4: Is 32768 correct, or should it be 32767? (I.e., a saturated 16-bit value?)

\rebut{You are right. The available ASIDs are between 1 and 32767.}

"It is believed that when an SEV VM is resumed with an ASID different from its own... crash" (p5). "Believed" by whom?

\rebut{This is an assumption made in the SEV whitepaper. We will add references. We have revised in the paper.}

I wasn't entirely sure if the Crossline attacks ever actually needed to use page-fault side channels, as described on p6. I got the impression that they do, but then the performance numbers are low and stable enough that I became unsure. Please clarify.

\rebut{No, Crossline attacks don’t need page-fault side channels. Crossline attacks directly learn the secret from the page fault’s physical address instead of the pattern of faults (as is the case in side-channel attacks). We will make this clear in the revision. }


Maybe call out the 2-seconds-to-decrypt-8-bytes as a naive solution as it is introduced, since an optimization follows very shortly?

The paper was pretty heavily focused on fingerprinting application binaries. Do you think it's not worth going fishing for data that happens to be formatted in a way to be compatible with PTE? Better to just get code execution? What about if extreme stealth was an attacker's goal?

\rebut{Extreme stealth is the one of the advantages of Crossline. For example, with only SEV-enabled VM (as google deployed), the platform host can scan and steal data from the VM with 0-risk.}

The paper dismisses a guest trying to detect an unexpected CR2 change as infeasible. Is this really true? What if the hypervisor took responsibility for sanitizing it sometimes?

\rebut{Similar Question from Review A.
}

\bheading{Minor}

s/nest paging/nested paging/ on p4 (s/needed/need/ later in the same sentence)

last sentence just before section V starts. s/until succeeds/until it succeeds/ (missing "it")

s/enabled a chosen plaintext/enabled chosen plaintext/ on p13

\rebut{We have revised them accordingly.}


\subsection*{\textcolor{Maroon}{Review C}}
\bheading{Overall recommendation:}
4. Minor revision

\bheading{Writing quality:}
3. Adequate

\bheading{Reviewer Confidence:}
3. Sufficient confidence

\bheading{Paper summary:}

The paper introduces two attacks on AMD SEV, named CrossLine V1 and V2. Both attacks are based on the fact that AMD SEV does not authenticate the VMCB, a control block that records part of a VM's state upon an exit to the hypervisor. The attacks specifically abuse the VMCB's ASID value, which identifies the VM to the CPU. The CPU uses the ASID to select a key from its secure co-processor that is going to be used to encrypt and decrypt memory requests. The attacks require a malicious VM colluding with the hypervisor to attack a victim VM. CrossLine V1 allows to dump a victim's VM memory by modifying the attacker's RIP so that at resumption, the attacker VM will try to access a particular offset of a page. It then remaps the page being requested to the victim's memory and replaces the ASID to the victim's ASID so that the page fetched is decrypted with the victim's key. The result is returned to the hypervisor by embedding it in a page fault error information. In CrossLine v2, the RIP value is chosen so that a mov from mem to reg is executed. As all the registers are present in the VMCB, the hypervisor can then know what value was in the memory location accessed. Similarly, if the RIP fetches a memory write operation, the attacker can modify the victim VM and hence tamper with its integrity in an undetectable way. The attacks only apply to AMD SEV, a partially (only V1) to SEV-ES, but not to SEV-SNP, the newest SEV proposal of AMD.

\bheading{Strengths:}

+ Interesting attacks.

+ Nice description of the internal workings of SEV.

+ The attacks were evaluated on real hardware.

\bheading{Weaknesses:}

- The description of the attacks is cumbersome to follow.

\bheading{Detailed comments for authors:}

I found the paper and the attacks interesting to read. The paper gives a good introduction into AMD SEV, and the paper can be followed even if the reader is not familiar with AMD SEV. That said, I think there are a couple of sections that could and should be improved, as the description of the attacks as it is now is not easy to follow.

You specify the vulnerability that you exploit security-by-crash’’. While I agree with the name, I do not fully agree with this as the sole reason. To me it seems like a pretty big oversight of AMD to allow modification of the ASID in between a VMEXIT and a VMRUN. If I understood the attacks correctly, any integrity verification on the ASID field would render the attack useless. Because of this, I would also add ``Unencrypted VMCB to the exploited vulnerabilities of CROSSLINE v1 in Table II. As such, I must notice that other previous attacks have taken aim at the same vulnerability and were able to achieve something close to CROSSLINE. However, CROSSLINE is stealthy.

\rebut{We agree. A secure design of SEV should protect ASID from malicious hypervisors. However, this is not a choice made by SEV/SEV-ES/SEV-SNP. Rather than protecting ASIDs from manipulation, SEV/SEV-ES/SEV-SNP relies on security-by-crash to ensure confidentiality and integrity of the VMs. It is our aim to clearly point out this oversight in this paper.
The reason behind this design choice is that ASIDs must be managed by the hypervisor. This is because the hypervisor is in charge of managing the lifecycle of VMs, including assigning an ASID to a newly launched VM and freeing the ASID of a terminated VM. Note it is also a choice made by Intel TDX.
}

In general, I do not understand why the authenticity check introduced in SEV-ES does not cover more fields of the VMCB. If you can argue why it cannot cover all fields, e.g., because the hypervisor needs them to handle faults, then your attack gets even stronger.


\rebut{Some fields in VMCB are unencrypted in SEV-ES/SEV-SNP, such as ASID, TLB-control field, EXITINFO, Nested CR3, etc., in order to support virtualization. The hypervisor is in charge of handling VMEXITs, extracting the faulting guest physical addresses from NPF’s EXITINFO, managing the pool of ASIDs for all VMs, etc. The encrypted VMSA does not include the ASID field.}

It is interesting how the proposed SEV-SNP could potentially mitigate the CROSSLINE attack, but I missed a section that discusses countermeasures. In other words, is there an easy way to mitigate the CROSSLINE attacks? And what would the downsides of such a mitigation be? More overhead? More production cost?

Writing: First, many terms get referenced often like the gCR3 or the NRIP or the SPFN0. It would be useful to have a table with all of these terms so that a reader can quickly look at it when these terms are mentioned.

Second, some AMD VM specific terms are never defined. For instance, VMEXIT is never clearly introduced, and it was unclear for me if it meant that the VM would be destroyed rather than just paused. The same holds for VMRUN.

Regarding the description of the attack steps, I think a better figure 3 would go a long way. As now, it's hard to follow what gets modified, when, and why. One possible way to make it clearer IMO could be to have a snapshot for each relevant step of the gCR3, the page table mappings, and the ASID so that by looking at the figure, it is clear where pages are being remapped and what values are being modified. A similar figure for CrossLine v3 should also be there.

\rebut{We move Crossline V3 to appendix since we failed to find an end-to-end attacks related to Crossline V3.}

Something else that is unclear until Section V is that the registers are also contained in the VMCB, but they are already assumed as available to the attacker in CrossLine V2. This fact should be said before as well.

Is the RIP of the VM contained both on the VMCB and the VMSA? Can you please be more clear about this in Section V.A1?

\rebut{In SEV-ES, both the (unencrypted) VMCB control area and the VMSA include the next RIP field. However, the next RIP field in the VMCB control area is masked with 0, which suggests RIP cannot be controlled by the hypervisor in SEV-ES. }

The intro should mention what the ASID is before using it.

\rebut{Thanks and we added the explanation in abstract. }

Typos:

with one standard deviation of -> with a
Sec V.C: encrypted VMCB -> did you mean VMSA?

\rebut{We have revised them accordingly.}



\subsection*{\textcolor{Maroon}{Review D}}
\bheading{Overall recommendation:}
2. Leaning towards reject

\bheading{Writing quality:}
3. Adequate

\bheading{Reviewer Confidence:}
4. High confidence

\bheading{Paper summary:}

This paper presents an attack called CrossLine against AMD SEV. Specifically, CrossLine turns the nested page fault into an oracle that reveals the plaintext of the encrypted guest VM's quadword which follows the format of a page table entry (PTE). CrossLine further leverages this primitive to construct decryption/encryption oracles by identifying memory load/store instructions.


\bheading{Strengths:}

+ An interesting way to repurpose nested page faults for leaking secrets

\bheading{Weaknesses:}

- Works only on SEV (and partially on SEV-ES).

- Can only read quadwords which look like an PTE.

- Writing is tightly coupled with the lowest-level details of AMD SEV.

\bheading{Detailed comments for authors:}

It is an interesting idea to convert nested page faults into an oracle for reading SEV-encrypted guest memory. However, I am not too excited about this attack for two main reasons. First, it appears that this attack can only be effectively applied to the original AMD SEV (and partially to SEV-ES), while major cloud providers are likely to skip the original SEV (e.g., Google's recent announcement of Confidential VMs is based on SEV-ES). The upcoming Intel TDX is not vulnerable to CrossLine because the hypervisor has no direct access to the nested page table responsible for translating the encrypted range of the guest physical memory. That being said, the real-world impact of the attack is likely to be small. Second, the requirement of the PTE-alike quadword limits the oracle's application to only a small portion of guest physical memory. The paper also acknowledges that the percentage of readable memory blocks is small for real-world applications.

The authors seem to skip an important limitation: the non-executable (NX) bit of the quadword to decrypt must be cleared because the memory access controlled by RIP is an instruction fetch. This confused me when CrossLine is applied to dumping the victim's page tables: if the selected page table entry is marked as NX, the page permission violation will inhibit a nested page fault from happening, and thus its content cannot be leaked. In addition, the description of "Reading Arbitrary Memory Content" in Section IV.A also skips the NX bit (bit 63). If the authors can workaround this limitation, the authors should add relevant details to the paper.

\newexp{We have added more details in Section 4.1.2. in this submission.}

When applying CrossLine to SEV-ES, it is unclear how the adversary can know the actual value of RIP and hence the page offset of the decrypted quadword (or PTE). In SEV-ES, RIP is encrypted and stored in VMSA upon a VMEXIT. Even the adversary can reuse the same VMSA to mount the attack, she can only know a quadword of the leaked value exists on the guest physical page, but I don't see how she knows which quadword (of the 512 possible quadwords) has that value.

\newexp{We add additional experiments in Section 5.2, which can help the adversary to learn the offset pointed by RIP.}

The introduction mentions it is a side effect of the RMP implementation that prevents CrossLine from applying to SEV-SNP. I do not agree with the authors on this point. RMP fundamentally blocks this attack because it limits how a system physical page can be used by the hypervisor. For example, RMP purposely disallows a system physical page belonging to a guest VM from being remapped to a different guest physical address of the same VM. This is exactly what CrossLine abuses to decipher the guest's encrypted memory (by remapping the guest page table root to a different system physical page). To the best of my understanding, RMP makes the access control policy applied to the potentially malicious hypervisor explicit, which overturns the "security-by-crash" principle used in the original AMD SEV.

\rebut{It depends on how it is viewed. The root cause of CrossLine is that the hypervisor is able to manipulate ASID and run an attack VM with the victim’s ASID. In the paper, we show it is an issue with SEV/SEV-ES, as they still allow the attack VM to perform address translation (which leaks data during nested page faults). With SEV-SNP, manipulation of ASID is still allowed, but CrossLine V1 does not work due to RMP checks. We are not able to explore other CrossLine variants as we don’t have SEV-SNP machines. We hope the publication of this paper will inspire fellow researchers to derive clever ways to workaround RMP checks in similar attack settings, when SEV-SNP becomes available (possibly next year).}

\subsection*{\textcolor{Maroon}{Review E}}
\bheading{Overall recommendation:}
3. Major revision

\bheading{Writing quality:}
3. Adequate

\bheading{Reviewer Confidence:}
3. Sufficient confidence

\bheading{Paper summary:}

This paper describes a novel attack on AMD's Secure Encrypted Virtualization (SEV), which Google recently announced as forming the basis of its "Confidential Computing" cloud product. While there have been a number of attacks on AMD SEV, many of these have been addressed by AMD. This attack breaks an assumption made by AMD: that a compromised hypervisor cannot profitably manipulate the VM ASIDs, because the VM will simply crash. However, the authors show that by carefully manipulating the VM ASIDs, an attacker VM can decrypt 8 bytes at a time (crashing each time) and eventually dump the page tables (CrossLine v1) and the use that to either modify or decrypt specific values in a VM's memory (CrossLine v2).


\bheading{Strengths:}

+ novel attack on AMD SEV.

+ not many papers looking at AMD processor security

+ valuable background and deep understanding of AMD SEV and use of ASIDs.

\bheading{Weaknesses:}

- lacks demonstration of a practical attack.

\rebut{We acknowledge that Crossline attacks cannot be directly used to perform an end-to-end attack like stealing a private key under SEV-ES mode. However, the capability of Crossline V2 under SEV mode (read/write arbitrary memory in a completely stealthy way) fundamentally breaks SEV's protection. If the attacker has the power to decrypt/encrypt arbitrary memory, she can do everything.  }

- fairly limited performance evaluation.

\rebut{We have added new performance evaluation especially for Crossline in SEV-ES.}


- no discussion of potential solutions.

\rebut{We are not aware of any software-based solution. We can add some discussion on potential hardware mitigations in the revision. }


- writing is very technically dense with a somewhat wandering narrative.

\rebut{We have revised the paper accordingly. }


\bheading{Detailed comments for authors:}

This paper provides an interesting and valuable tutorial of AMD SEV and the intricacies of how the ASID is managed by the hypervisor. Though this, and much of the paper, is technically very dense and hard to follow. I suppose (if correct --- I can't check it) it will provide a valuable resource for academic security researchers who are not able to dive into the AMD technical specifications, or at least get a high level overview before doing so.

The attack itself is novel. I like that it does not overly rely on side channels or speculative execution. There has also been only a handful of academic papers targeting AMD architectures (though there have been several at top conferences in the last year or so) and it is useful to get some diversity from the traditional Intel focus of these papers.

I was, however, disappointed with the demonstration of the utility. The paper stops with: (a) we dumped the page table, and (b) we modified / retrieved some values from sshd. How much harder would it be to steal a symmetric or private key from the VM and then decrypt SSH traffic? Show the full utility of the attack. I would really like to see this in a major revision.

I don't have a good feel as to how scalable the attack is:

It seems to require a lot of manual inference about the victim VM and process in the victim VM. How automated can this get? I understand that some manual steps are needed, but this should be made clear.

\rebut{For Crossline V1, no manual inferences are needed.
For Crossline V2, we have demonstrated an automated attack that locates decryption/encryption instructions in sshd in around 0.5s. The adversary can automate the read/write of the guest VM’s memory afterward. 
}

Rebuttal indicates V1 no manual inference and V2 gets it in around 0.5s. I don't think you got my question. How much manual effort did you take in tailoring your attack for sshd? You had to know a lot about the binary and memory structure to make the attack useful. This is what I thought should be clarified.

\rebut{For Crossline V2, the adversary needs to help some pre-knowledge of sshd binary. However, since Crossline V2 is completely stealthy, the attacker can repeat the steps until finding a useful instruction.}

I don't have a good feel for how long a practical attack would take. There are some good examples for the CrossLine v1 attack, including the VMCB rewinding optimization. However, I'd really like to see a macro-level performance evaluation towards the end of the paper, putting everything together.
The narrative of the paper could also use work. It currently reads as:

We made the CrossLine v1 attack. It got us the page tables, but we really couldn't get much useful out of reading process memory, because less than 7\% of the data was 8-byte aligned. So, we created these oracle things. That seems useful, and look, these small tests show we can read and write 8-byte values. Oh, and after we did this, we thought we should look at whether or not AMD SEV-ES had any impact. It does, but here's how we got around that. And then after we wrap everything up, here's a new variant that we came up with after writing most of the paper. We thought you would think that is cool too, so we threw it on the end.

Finally, the paper is missing recommendations for fixing the problem. My intuition is that "security-by-crash" may still work if SEV can (a) prevent the duplicate ASID assignment, and (b) invalidate the KEK for an ASID in the AMD SP under certain conditions (e.g., on DEACTIVATION, or other edge conditions that are needed for the attack, but are not needed in normal operation).

Other Notes:

Reference [26] is missing the booktitle. This was IEEE S&P 2020.

\rebut{Thanks for these suggestions. We have revised them accordingly.}

==> 99-app.tex <==

\newpage
\onecolumn
\setcounter{page}{1}

\begin{center}
   {\Huge \textbf{Prior Reviews and the Author's Response}}
\end{center}

%The previous version of this paper has been submitted to USENIX Security 2020 and NDSS 2021. For USENIX Security, we received a decision of *major revision* (with two *accepts* from expert reviewers, three *major revision* from knowledgeable or ``some familiarity'' reviewers). For NDSS, we received a decision of *reject* (with two *minor revisions*, two *major revisions* and one *Leaning towards reject*). 
%We have revised our paper according to the suggestions (which are greatly appreciated) and added several new experiments in our revision, which are highlight in red.

\noindent We have submitted this paper to prior conferences and received very constructive feedbacks. In the following, we would like to present two sets of verbatim reviews (from USENIX Security 2020 and NDSS 2021 respectively) and describe in greater details of how we have addressed each of the comments. Particularly, we have revised our paper according to the suggestions (which are greatly appreciated) and added several new experiments (which are highlight in red) in our response.

%\setcounter{section}{A}
\section*{1. Previous Reviews (Usenix Security 2020)}

%\textbf{The previous version of this paper has been submitted to USENIX Security 2020 and NDSS 2021. For USENIX Secureity, we received a decision of *major revision* (with two *accepts* from expert reviewers, three *major revision* from knowledgeable or ``some familiarity'' reviewers). For NDSS, we received a decision of *reject* (with two *minor revisions*, two *major revisions* and one *Leaning towards reject*). 
%We have revised our paper according to the suggestions (which are greatly appreciated) and added several new experiments in our revision, which are highlight in red.} 


%\textbf{We have attached the verbatim reviews from USENIX Security 2020 and NDSS 2021 below and interleaved with our response to the comments.}

\subsection*{\textcolor{Maroon}{Review A}}

Missing for unknown reasons.

\subsection*{\textcolor{Maroon}{Review B}}
\bheading{Review recommendation:}
5. Accept

\bheading{Writing quality:}
4. Well-written

\bheading{Reviewer interest:}
3. I would definitely go to this talk and tell my students or colleagues to read this paper

\bheading{Reviewer expertise:}
4. Expert

\bheading{Paper summary:}

This paper introduces the CROSSLINE attacks that can compromise the confidentiality and integrity of SEV-enabled VMs on AMD platforms. The paper investigates the ``security-by-crash" principle behind the design of SEV and shows that a malicious hypervisor can launch an attacker VM that temporarily executes a few operations in the context of a victim VM before a crash. These operations allow the hypervisor to leak sensitive information and compromise the integrity of the victim VM.

The paper builds three variants of CROSSLINE. CROSSLINE-v1 relies on nested page faults to incrementally build the state of the victim VM's page tables. CROSSLINE-v1 can further leak sensitive contents that have the format of page table entries. CROSSLINE-v2 executes actual instructions in the context of the victim VM that can leak memory contents from registers (read by the hypervisor after a VMEXIT through VMCB) or overwrite memory contents by using store instructions with the provided register contents. CROSSLINE-v3 shows that the attacker VM can reuse TLB entries of the victim VM, simplifying v2 exploitation without preparing page tables in the attacker. The lack of checks in the TLB can potentially allow compromising the future SEV-SNP VMs.

\bheading{Strengths:}

+ Novel attacks against AMD-SEV

+ Proof of concept exploits with evaluation

+ Clear presentation

\bheading{Weaknesses:}

- Impact is similar to previous work

\rebut{The consequences may be similar, but the security implications are different. Compared to these prior works, CrossLine explores a different problem in the SEV design (i.e.,“security-by-crash”). While the design of SEV-SNP is motivated by these prior works, it is clear that the vulnerability exploited by CrossLine was not the primary consideration of SEV-SNP and thus it may lead to other attacks. Moreover, Crossline cannot be detected by the victim VM, because it does not make use of any data structure of the victim VM (such as VMCB, NPT) or alter its control flows. Crossline will change how researchers design software-based defenses against previously known attacks. For example, our paper shows it is meaningless to design a detection system that runs in the victim VM to detect misbehavior of the hypervisor.} 

\bheading{Detailed comments for authors:}

This is an interesting work exploring the security implications of allowing an untrusted party to execute instructions in the context of an SEV-enabled VM. The developed attacks are novel with clear explanation and evaluation. From an impact point of view, compared to previous work, perhaps the most interesting variant is CROSSLINE-v1 that is also effective against SEV-ES. The paper can improve with a table that compares the impact of CROSSLINE variants and past work on different SEV versions.

\rebut{We have included such a table (\tabref{table:attacks}) in \secref{sec:related}.}

I was surprised that CROSSLINE-v1 on SEV-ES VMs leaves no trace, specially given that a triple fault modifies the VMCB. The paper should discuss why the victim VM can continue gracefully when started with a triple fault without leaving any trace.

\newexp{We have included additional experimentation to explain this in \secref{sec:counter:seves}.}

I really liked that the authors evaluated CROSSLINE-v1 on different applications for the old SEV version. The same attack also works for SEV-ES, but I would expect that the leakage is more limited due to lack of control over the instruction pointer. It would be good if the authors report the leakage percentage for SEV-ES as well.  

\newexp{We have included extra experiments in \secref{sec:counter:seves} to show how the adversary could improve \atknameOne on SEV-ES.}
%\rebut{In theory, the leakage percentage for SEV-ES is the same as SEV, with the only difference being the lack of control of nRIP and hence the page offset. Note the attack can be performed on any level of the page tables; therefore bits 47-39, 38-30, 29-21, and 20-12 of the same RIP can all be used as the page offset by the attacker. Therefore, with any RIP, there are 1~4 different offsets that the attacker may use to extract data on any encrypted page. As there are only 512 possible page offsets (as PTEs are 8-byte aligned), repeating the attacks with different RIPs multiple times would likely to cover a large fraction of offsets. In theory, assuming random RIPs and each leads to one offset, to cover all 512 offsets, roughly 512*ln(512)+γ*512+0.5 = 3500 RIPs are needed to decrypt all pages (see Coupon Collector Problem). Of course, RIPs cannot be completely random, so we expect a bit higher effort in practice. We have included additional experiments to validate this point in this draft.}

Some minor presentation issues: in 4.2.1, the immediate examples are not clear. It is better to first explain the masks, before explaining how the page fault address can translate to the data. 

Nits: All VEKs .. is never, nest paging, to invalid.

\rebut{revised accordingly.}


\subsection{\textcolor{Maroon}{Review C}}

\bheading{Review recommendation:}
3. Major revision

\bheading{Writing quality:}
4. Well-written

\bheading{Reviewer interest:}
2. I might go to a talk about this

\bheading{Reviewer expertise:}
3. Knowledgeable

\bheading{Paper summary}

This paper shows, that AMD's use of ASIDs to map SEV encryptions keys to VMs, is flawed. According to the SME Whitepaper AMD argues that while the ASID used by a VM is under control of the hypervisor, running an SEV secured VM with a different ASID immediately leads to a crash. However, as shown in the paper, a malicious hypervisor can carefully craft an attacker VM that is able to read and write data data encrypted with another VM's memory encryption key. The paper presents three attack variants. The first one exploits that nested page faults leak the GFN of the fault to the hypervisor. The second and third variant execute instructions under the victim VM context and leak data to the general purpose registers, which are stored in the VMCB on VMEXIT. The first attack also works with SEV-ES, although the control over the RIP register is reduced.

\bheading{Strengths:}

+ Novel attack angle, that does not rely on SEV's missing integrity protection

+ Victim VM does not need to run concurrently

\bheading{Weaknesses:}

- CrossLineV1:
Under SEV-ES, the attackers control over the decrypted memory location is more restricted as the the page offset cannot be chosen directly. In addition, the data must conform to the PTE format to be leakable.

\newexp{We have added experiments about the adversary's capability of reaching different page offsets and the results show several minutes are sufficient to reach all 512 offsets. Even though the data must conform to the PTE format to be leakable, it is useful to identify or learn memory content, dump process's page table and break ASLR or KASLR, which already breach SEV or SEV-ES's security guarantees.}

- CrossLineV2 and CrossLineV3: 
Under SEV-ES the general purpose registers in the VMCB are encrypted and thus can no longer be used by an attacker to move data into/out of the victim VM. The authors do not describe, an alternative approach that allows to read or write data with these attacks in the SEV-ES context.

\rebut{We have discussed the limitation of \atknameTwo in this draft.}

\bheading{Detailed comments for authors:}

I really like the novel approach of your paper. However, in my opinion, its security implications for SEV-ES are not very strong. With CrossLineV1 the attacker has limited control over the data, that he is able to read. While he can choose the page frame number, the page offset is determined by the RIP value of the victim VM. With SEV-ES, the attacker can only indirectly manipulate this value by trying to stop the VM at a fitting offset. Repeating the attack many times, the attacker should still be able to generate every page offset.

CrossLineV1 can only leak data from 8 Byte aligned addresses, whose content conforms to the PTE format. For CrossLineV2 and CrossLineV3, leaking data into the general purpose registers is no longer possible under SEV-ES (as they are encrypted with the victims VEK on a #VMEXIT). In my opinion, this (mostly) mitigates these two variants. I would like to see a more severe attack, e.g. reading/writing arbitrary data or  extracting sensitive data, like encryption keys, with a high success probability (given the data data format restrictions of CrossLineV1). 

\rebut{CrossLine V1 can be used to dump the guest VM’s page tables, which can be used to break (K)ASLR. With the efforts described above, it also works on SEV-ES. It can also help fingerprinting binaries, which does not always need the attacker’s fine control of the fitting offset.}

``4.2.1 Constructing Decryption Oracles'': In order to find suitable instructions for CrossLineV2 and CrossLineV3, you suggest using CrossLineV1. Where you able to reliably find such instructions this way (given the low amount of leakable memory)? Otherwise, writing
``We make no assumption of the adversary's knowledge of the victim VM, including its kernel version, the applications running in it, etc." 
is a bit misleading.

\rebut{We meant the attacks do not rely on a specific kernel version, but knowledge of such information does improve the quality of the attack. We have revised this paragraph accordingly.} 

nRIP and RIP:

What is the connection between nRIP and RIP? The description of the CrossLineV1 attack under plain SEV suggests that the value of nRIP is used for RIP after resuming the VM. I was unable to find Documentation for that. 

\rebut{We have added references in our revision.}

If this is the case, how does this relate to the following sentence?
``... the attacker VM cannot change the register values that are stored in the VMSA, which includes RIP,... . Therefore, with SEV-ES, the adversary is no longer able to arbitrarily control the execution of the attacker VM by simply manipulating its nRIP in its VMCB's control area."

Does the VM simply ignore the value of nRIP in the SEV-ES case?

\rebut{According to AMD64 Architecture Programmer’s Manual Volume 2: System Programming[2] (15.7.1 State Saved on Exit), “the next sequential instruction pointer (nRIP) is saved in the guest VMCB control area at location C8h” and “the nRIP is the RIP that would be pushed on the stack” during VMRUN. This also applies to SEV. However, SEV-ES encrypts the VMCB. There is an RIP field in the VMSA (encrypted), which will be advanced automatically during VMRUN (described in section 15.35.4 “Types of Exits” [2]) and then used as the instruction pointer. In our experiments, for SEV-ES, the nRIP in the VMCB control area (unencrypted) is always 0 during VMEXIT.}

``This could work because the attacker VM has not successfully fetched a single instruction yet;" :

Is ``could work" a typo? The context suggest that the described attack *actually* works.

\rebut{The attack actually works. We have changed the wording.}

Typos:

``...distinguishes different VEKs using ASID" $->$ "...distinguishes different VEKs using ASIDs"

``...ASIDs are used by AMD-SP" $->$ "...ASIDs are used by the AMD-SP"

``...few instructions encrypted with victim VM’s VEK." $->$ "...few instructions encrypted with the victim VM’s VEK."

``...Then next NPF VMEXIT reveals..." $->$ " Then, the next NPF VMEXIT reveals..."

\rebut{We have revised them accordingly.}

\bheading{Requested changes:}

- Provide a more severe attack for SEV-ES, e.g. reading/writing arbitrary data or leaking sensitive data, like encryption keys, with a high success probability.

\rebut{Leaking crypto keys is a common goal in side channel attacks, but may not be a proper target in this context. We believe under the threat model of SEV, leaking any encrypted data is already considered a severe attack. }

\bheading{Questions for authors' response:}

- Why do you think the attacker for SEV-ES can be used to extract useful information?

\rebut{Even \atknameOne is more limited in SEV-ES due to the lack of control over the instruction pointer, we show it is easy to stop the victim VM at all 512 offsets. By doing this, the adversary can dump guest VM’s page tables and break KASLR and ASLR. The adversary can also have a knowledge of guest VM’s memory (the percentages of 8-byte memory blocks that can be directly read varies from 1.0\% to 6.5\%), which will be enough for fingerprinting binaries in memory. }

- How are your CrossLineV2 \& CrossLineV3 attacks for SEV an improvment over the "unencrypted VMCB" attacks from Buhren et al. [9] and Werner et al.[25].

\rebut{Compared to these prior works, CrossLine explores a different problem in the SEV design (i.e.,“security-by-crash”). While the design of SEV-SNP is motivated by these prior works, it is clear that the vulnerability exploited by CrossLine was not the primary consideration of SEV-SNP and thus it may lead to other attacks. Moreover, Crossline cannot be detected by the victim VM, because it does not make use of any data structure of the victim VM (such as VMCB, NPT) or alter its control flows. Crossline will change how researchers design software-based defenses against previously known attacks. For example, our paper shows it is meaningless to design a detection system that runs in the victim VM to detect misbehavior of the hypervisor.}
 


\subsection*{\textcolor{Maroon}{Review D}}


\bheading{Review recommendation:}
3. Major revision

\bheading{Writing quality:}
2. Needs improvement

\bheading{Reviewer interest:}
3. I would definitely go to this talk and tell my students or colleagues to read this paper

\bheading{Reviewer expertise:}
3. Knowledgeable

\bheading{Paper summary}
The paper presents CrossLine, an attack on AMD’s SEV technology. At a high level, SEV allows encrypting VMs memory, such that even a malicious hypervisor is unable to read the VM’s memory. To achieve this, each VM is assigned a unique ASID, which controls which encryption keys are used to decrypt and encrypt the VMs memory using a hardware encryption engine inside the CPU. While the hypervisor can modify the ASID of an attacker VM, it is assumed that since the memory will be decrypted with a wrong key, the modified VM will crash. 

On the other hand, the authors show that in case an attacker VM is assigned the ASID of a victim VM, the page table walker is able to perform a walk before the inevitable VM crash due to the wrong keys being used. This allows the authors to decrypt part of the victim’s page table, and in fact any 8-byte aligned memory address that conforms to a PTE format (about 1.5\% of memory). Next, leveraging this together with a gadget in the victim VM, the attacker is able to obtain an ability to dump the entire memory contents of the victim VM. Finally, in a third result, the authors show how to execute a few instructions of the victim VM by the attacker before a crash.

\bheading{Strengths:}

+ The topic is a good fit for a venue like Usenix, especially since the security of AMD’s architecture is far less studied compared to Intel’s.

+ The result is nice, and is basically a breach of SEV’s security guarantees. The fact that the authors can passively decrypt some memory and dump the entire VM via a gadget is impressive.

+ From a technical perspective, I like how the authors build the decryption oracle for the second attack from the first attack that is able to decrypt PTE. Moreover, even by itself the first attack is clever, and has some nice tricks against the AMD architecture.

\bheading{Weaknesses:}

-	The paper can use an editorial pass and a gentler introduction to SEV. The current version simply throws a lot of technical AMD details at the reader, which I personally had a hard time following at points.

\rebut{Thank you for your suggestion. We have accordingly revised the introduction and made it a bit gentler. }

-	To dump the VM memory the attack needs a gadget in the victim VM while the passive attack can only dump about 1.5\%. Yet, the authors do not demonstrate the existence of such a gadget in Linux, nor do they demonstrate the extraction of secrets in the 1.5\% of memory that they can passively decrypt.

\newexp{We added an end-to-end attack to show how the adversary can find such gadgets.}

-	The next generation of SEV (SEV-ES and SEV-SNP) stop most of the proposed attacks. In particular it is quite obvious that encryption without authentication (i.e., security by crash) will not have a good outcome.

\rebut{``encryption without authentication" and ``security-by-crash" are two fundamentally different concepts.}

\bheading{Detailed comments for authors:}

Thank you for submitting to Usenix Security, I like the topic you consider and I enjoyed reading your paper. The result is nice, as it effectively breaches the confidentiality guarantees of AMD’s SEV. I like the technical tricks in the first attack and how you abused the page table walker to decrypt any PTE-like memory region. The fact that the second attack is able to use a single instruction gadget to dump the entire VM is further contribution. This is a nice and impactful result.


On the negative side, the paper can use some additional editorial work and a gentler introduction to SEV. Right now, the paper throws a lot of details and initials at the reader at a very fast pace, making the paper hard to follow. Next, at points the paper oversells its results. For example, in Section 1 the paper claims that CrossLine is able to extract VM memory without the victim running. However, it was very disappointing to find out that this is true for ~1.5\% of memory, requiring not only interaction with a victim but also a code gadget to extract the rest. While the result is nice, toning down the language and improving the SEV and attack description will significantly improve the paper’s readability. 

\rebut{Thank you and we have toned down our language.}

Next, speaking of code gadgets and memory decryption, the paper does not show the extraction of secrets (e.g., keys, user input or data) in the 1.5\% of memory you can passively decrypt. Showing this will make the attack stronger. Similarly, while the code gadget required for the second attack is super simple (a single instruction), the paper does not say if such a gadget was found in a natural installation. Showing an end-to-end attack for the second variant will make the paper stronger. 


\newexp{We have included  an end-to-end in \atknameTwo and show how the adversary is able to locate an encryption and a decyrption instruction within 500ms. }

Finally, at a high level it is quite obvious that without authentication, AMD’s “security via crash” approach will fail somehow. The fact that future generations of SEV added authentication and generally prevent the presented attack does reduce the paper’s impact. 

Overall however, I like the work and I think this should be published. My recommendation is a major revision, asking the authors to improve the paper’s editorial quality, show and end-to-end attack using the second variant in a natural installation, as well as demonstrate extraction of secrets using the first variant (if possible).

\bheading{Requested changes}

Please improve the following for the next version:

1.	Make an editorial pass on the paper and give a gentler introduction to SEV and a more high-level attack description. Throwing technical details at the reader makes the paper hard to follow. In addition, please tone down the language of the paper’s claimed contributions (the interaction with the victim VM mentioned above is only one example of overselling). 

\rebut{We have revised these accordingly. Thank you for your suggestion.}


2.	Demonstrate an end-to-end attack using the second variant, by finding the suitable code gadget in a natural installation on a VM without any modifications.

\newexp{We have demonstrated such an end-to-end attack}

3.	If possible, demonstrate the extraction of some secret data (keys, user data, user inputs, etc.) using the first variant of the attack.



\subsection*{\textcolor{Maroon}{Review E}}

\bheading{Review recommendation:}
3. Major revision

\bheading{Writing quality:}
4. Well-written

\bheading{Reviewer interest:}
2. I might go to a talk about this

\bheading{Reviewer expertise:}
2. Some familiarity

\bheading{Paper summary:}
This paper introduces Crossline, a new family of attacks of SEV, a feature of recent AMD CPUs that aims to protect the confidentiality and integrity of guest VM memory from a potentially malicious hypervisor. SEV works by encrypting a each guest VM's memory pages under a different key that stored in the CPU that is never revealed to the hypervisor. Each guest VM is assigned a unique ID, called an ASID. The CPU uses the ASID to keep track of which key to use to decrypt the VM's pages.

The paper identifies a potential weakness in SEV: the untrusted hypervisor is responsible for assigning ASIDs to VMs, and a malicious hypervisor could change a colluding attacker VM's ASID to match that of a victim VM. This would cause the CPU to start using the same memory encryption key for both VMs. As the paper points out, SEV seems to assume that switching an attacker VM to use a victim VM's key will not cause problems because the attacker VM will crash as soon as it tries to decrypt its own memory with the wrong key.

Crossline attacks undermine this assumption because, as the paper shows, although the attacker VM does crash, it is able to read or modify some of the victim VM's memory beforehand. The paper presents three variants of the attack:

- V1: The malicious hypervisor sets up the attacker VM's address space so that when the attacker VM runs with the victim VM's ASID, it generates a page fault before crashing. The faulting address, which is revealed to the hypervisor, can be made to actually contain 8 bytes of the content of the victim's memory. This process can be repeated to leak an entire 4KB page in ~40ms. The 8 byte block being leaked must match the format of a page table entry, and so, in practice, only about 1--2\% of a victim's code pages can be leaked in this way. The attacker can learn the victim VM's entire page table, however, which might help with subsequent attacks.

- V2: The malicious hypervisor sets up the attacker VM's address space so that when the attacker VM runs with the victim VM's ASID, the CPU decrypts and executes a few instructions from the victim's memory. These instructions could read from the victim's memory into registers, which are visible to the hypervisor as part of the VM's saved context. This process can be repeated to leak the victim's memory at the rate of ~114ms/4KB page or even to write to the victim's memory if the instructions copy from registers to memory.

- V3: The malicious hypervisor sets up the attacker VM so that when the attacker VM runs with the victim VM's ASID, the CPU decrypts and executes a few instructions from TLB entries belonging to the victim. The paper does not present detailed results for this version of the attack, but provides anecdotal evidence that it works and speculates that it would function like V2 but without having to modify the attacker VM's page tables.

In all cases, the victim VM does not need to be running concurrently in order to exfiltrate or modify its memory, and so it has no opportunity to detect the attack in progress.

The paper concedes that recent improvements to SEV (SEV-ES and the subsequent SEV-SNP) at least partially mitigate Crossline attacks. SEV-ES appears to block V2, and it seems to slow the more limited V1 attack down by ~2 orders of magnitude. Moreover, SEV-SNP seems to block V1 entirely. The paper speculates that V3 would still work, but it cannot present definitive results because SEV-SNP CPUs are apparently not yet available.

\bheading{Strengths:}

1. Crossline appears to be a new family of attacks on AMD SEV that cleverly exploit a questionable CPU design choice: an untrusted party can modify a security-critical label. It differs from prior attacks because it does not rely on SEV's lack of memory integrity protection, nor does it rely on speculative execution.

2. The paper demonstrates that Crossline V1 and especially V2 are practical and can exfiltrate a victim VM's memory at a relatively high rate.

3. The paper well-written and clearly explains Crossline's three variants.

\bheading{Weaknesses:}

1. The paper does not present detailed results on the effectiveness of Crossline V3. It only discusses a single example that seems to indicates that the attack will probably work.

\rebut{We move V3 to discussion and treat it as a proof-of-concept extension.} % Making V3 an end-to-end attack require considerable engineering efforts, which we hope to leave to future work.}

2. Subsequent revisions to SEV seem to be chipping away at Crossline's effectiveness. By the time CPUs with SEV-SNP are available, only V3 might still work, and even that has not been confirmed.

\rebut{While the two demonstrated \atkname variants may not work on SEV-SNP, the security flaws it exploits remain unfixed. Other variants like V3 may be discovered and confirmed when SEV-SNP processors are available.}

%\rebut{By the time we submitted \atkname to AMD team, the SEV-SNP is not published yet. Moreover, the SEV-SNP is a special version of SEV, which may cause performance downgrading. Customers themselves may choose to use SEV or SEV-SNP. It is meanful to help the designer realize the fundamental ``secure-by-crash'' problem in SEV series.}

3. The paper does not explain whether or not Crossline attacks are fundamental and how hard they are to mitigate. Are Crossline attacks part of a broader class that will be with us for a long time like speculative execution attacks, or are they AMD-specific bugs that could be fixed in the next revision of SEV?

\rebut{We have revised the introduction to reflect some of the ideas here.}

%\mengyuan{The ``security-by-crash" is one of the basic design in SEV and that untrusted hypervisor has fully control over ASID, which is trusted by hardware.}

\bheading{Detailed comments for authors:}

Overall, due to weaknesses \#2 and \#3, the paper's current state makes it hard to evaluate the significance of Crossline attacks. The fact that the newest version of SEV already mitigates V1 and V2 makes one doubt that the attacks are deep. Furthermore, AMD seems to have developed these mitigations independently. If that is the case, then this paper was not responsible for those improvements. Finally, it is unfortunate that the one Crossline variant that may still work against SEV, V3, is not well fleshed out in the paper.

Typos:

- p.7, bottom of 1st col: s/a 8-byte memory block/an 8-byte memory block.

\rebut{revised.}

- p.8, top of 1st col: s/tirals/trials.

\rebut{revised.}

- p.9, 4.2.2, last work: Should this be 1s instead of 1ms?

\rebut{1ms is correct. The time needed to encrypt 4KB memory page is around 100ms. But in a real attack, the adversary may only need to alter several bytes to compromise the victim VM. Then the time needed to launch a real attack should be done within 1ms.}

- p.11, last word of 1st col: s/invalid/invalidate

\rebut{revised.}

- p.13, first full paragraph: s/response to network requests/respond to network requests

\rebut{revised.}

\bheading{Requested changes:}

- Discuss how fundamental Crossline attacks are and how hard they would be to mitigate completely.

\rebut{revised.}

- Evaluate Crossline V3 experimentally in detail as the paper currently does with V1 and V2.

\rebut{We have moved V3 to appendix. A comprehensive end-to-end evaluation of V3 requires new techniques to learn the victim's virtual address space, which is not the focus of this work. }

- Confirm experimentally that Crossline V3 works against SEV-SNP. (Admittedly, this would require waiting until CPUs with SEV-SNP are available.)

\rebut{We withdrew the paper in respond to this request.}

- If AMD's mitigations were developed in response to this work, please do mention it.

\rebut{revised.}

\subsection*{\textcolor{Maroon}{Review F}}


\bheading{Review recommendation:}
5. Accept

\bheading{Writing quality:}
5. Outstanding

\bheading{Reviewer interest:}
3. I would definitely go to this talk and tell my students or colleagues to read this paper

\bheading{Reviewer expertise:}
4. Expert

\bheading{Paper summary:}
This paper presents a set of elegant attacks on AMD SEV. The attacks ignore the other problems of SEV and focus on the "security-by-crash" approach. The insights of the work are relevant, as they show that a "security-by-crash" design is principally broken.

\bheading{Strengths:}

- Well written

- Elegant and novel attack

- Practical impact and clear insights

\bheading{Detailed comments for authors:}
I really enjoyed reading this paper. The writing quality was really good, except for a handful of typos.
Section 3 gives a very good overview on the basic security-by-crash design and already gives the reader an intuition of what will go wrong.

Attack variant 1 is quite elegant. In Section 4.1.1, I'm not sure though why the slow results without VMCB rewinding are presented at all? Do they have an advantage, like a difference in detection possibility? What was the standard deviation for the 39.58ms?

\rebut{Revised accordingly. The average time of decrypting 4KB memory page is 39.58ms with one standard deviation of 4.26ms. }

Attack variant 2 is more straight-forward. For the encryption "oracle". Does the victim VM indeed pick up the corrupted values?

\rebut{Yes, the adversary is able to change any memory block inside victim VM.}

The explanation for attack variant 3 appears is only a theory without a proof in this paper. Maybe you could prove your theory by evicting/flushing the TLB entries and analyzing how that affects the attack? Otherwise make sure to label it as a theory consistently throughout the paper.

Discussion of applicability to SEV-SNP and the relation to speculative execution attacks makes sense, although Spectre is the only actual speculative execution attack in that list.

Please make sure that AMD is fully aware of your attack by obtaining a response statement from them, and will have security advice or patches before the publication of the paper.

\rebut{Yes, and the paper has been revised accordingly.}

\subsection*{Comment @A1}

The paper results in a vivid discussion among the reviewers. They all found merit but would want to see the following items addressed in a major revision:

* Improve the writing as outlined in the reviews.

\rebut{revised.}

* Mention limitations upfront to avoid raising the impression of overselling

* Evaluate V3 experimentally on SEV and demonstrate end-to-end attacks for V2 and V3 in a realistic scenario (e.g., leaking a crypto key).

\newexp{We have added an end-to-end attack example for V2 in Section \ref{sec:attacks}. We have moved V3 to Section \ref{sec:discuss}.}

* Evaluate the extraction of the victim's memory (as opposed to its page tables) using V1 on SEV-ES. Discuss/show other possible attacks using V2 and/or V3 on SEV-ES.

\rebut{We have extended our discussion on the faction of application memory that can extracted by \atknameOne.}
\newexp{We have added experiments about how the adversary can cover all 512 offsets in a short time in Section \ref{sec:countermeasure}. }

* Clarify whether AMDs mitigations were developed in response to this work or independently.

\rebut{Revised.}

* Discuss the arms race around SEV and how fundamental Crossline attacks are and how hard they would be to mitigate completely.

\rebut{Revised.}

==> app-ccs.tex <==
\appendix
\section{Appendix: Reusing Victim's TLB Entries}
\label{sec:discuss:v3}

As extensions of the two attack variants, we also discuss (1) another variant of \atkname, which allows the attacker VM to reuse the TLB entries of the victim VM for address translation and execute some instructions, even without any successful page table walks; 


%\label{sec:appendix}
%\subsection{A New Variant: Reusing Victim's TLB Entries}
%\label{sec:discuss:v3}

First, we discuss a proof-of-concept attack that extends the other two variants. In particular,
in this attack, we show that the ASID-based TLB isolation can be breached. 
There were two VMs involved: the victim VM is an SEV VM whose ASID is 1; the attacker VM is a non-SEV VM whose ASID is 16. Both VMs only have one VCPU, which are configured by the hypervisor to run on the same logical CPU core. We assume the victim VM executes the following code snippet: 

\begin{lstlisting}[language=Python,basicstyle=\small]
 d83:41 bb e4 07 00 00   mov    $0x7e4,%r11d
 d89:41 bc e4 07 00 00   mov    $0x7e4,%r12d
 d8f:0f a2               cpuid  
 d91:eb f0               jmp    d83 
\end{lstlisting}

Specifically, the code updates the values of {\tt \%r11d} and {\tt \%r12d}, and then executes a {\tt CPUID} to trigger a VMEXIT. Following the common steps of \atkname, the adversary launches an attacker VM, changes its ASID during VMEXIT, sets the \nrip of the attacker VM to the virtual address of the code snippet above, changes offset 090h of VMCB to make it an SEV VM, and resumes the attacker VM. Unlike \atknameOne and \atknameTwo, the nPT of the attacker VM is not changed in this step. Therefore, if the attacker VM performs a page table walk, a NPF will be triggered.\looseness=-1

Interestingly, the execution of the attacker VM triggers {\tt CPUID} VMEXITs before a triple fault VMEXIT crashes it. Since no NPF is observed, the attacker VM apparently does not perform any page table walk.
However, during the attacker VM's  {\tt CPUID} VMEXITs, we observe that the values of {\tt \%r11d} and {\tt \%r12d} have been successfully changed to {\tt \$0x7e4}. It is clear that the two MOV instructions and the subsequent  {\tt CPUID} instruction have been executed by the attacker VM. This is because the attacker VM was able to use the victim VM's TLB entries left in the TLB to translate the virtual address of the instructions. The triple fault might be caused by code executed outside the page, whose translation is not cached in the TLB.

While the consequences of this attack are close to V2, it highlights the following flaws in AMD's TLB isolation between guest VMs: (1) ASIDs serve as the only identifier for access controls to TLBs, which can be \textit{forged} by the hypervisor, and (2) TLBs cleansing during VM context switch is performed at the discretion of the hypervisor, which may be \textit{omitted} intentionally. 




% \mengyuan{maybe we just remove the MKTME}
% \subsection{Intel MKTME}
% %\bheading{Intel MKTME.} 
% Similar to AMD's SEV, Intel's Total Memory Encryption (TME) and Multi-Key Total Memory Encryption (MKTME)~\cite{intel:2019:mktme} also provide memory encryption to software.
% The concept of TME is similar to AMD SME: a memory encryption engine is placed between the direct data path and external memory buses, which encrypts data entering or leaving the SOC using 128-bit AES encryption in the XTS mode of operation. MKTME is built atop TME and supports multiple encryption keys. When used in virtualization scenarios, MKTME is close to AMD's SEV. However, different from SEV, where each VM only possesses one encryption key, multiple keys can be used in each VM on an MKTME platform, allowing cross-VM memory sharing when the same keys are used. The selection of encryption keys is controlled by software, by specifying the key id in the upper bits of a page table entry (PTE). In a virtualization scenario, the hypervisor has to be trusted because it has the capability of mapping guest VM's memory and controlling the memory encryption keys in the PTE. \atkname is not needed in the MKTME setting as a malicious hypervisor may directly read encrypted guest memory. Therefore, the hypervisor is included in the TCB of MKTME, which could greatly limit its real-world adoption. 

==> backup.tex <==
\section{Background}


\yz{The following paragraph has been proofread, but it does not seem to be relevant.}
The memory encryption engine uses a 128-bit AES key to encrypt data under the Electronic Codebook (ECB) mode of operation for performance concerns~\cite{du:2017:secure}. Each 128-bit aligned memory block is encrypted independently. An additional system physical address-based tweak function is used to prevent attacker from inferring memory block content in different physical address. The tweak function is defined as $T(A) = \bigoplus_{A_i=1}^{1 \le i \le 128}t_i$, where $A_i$ is the $i$th bit of system physical address $A$, $\bigoplus$ is the bitwise exclusive-or (\ie, XOR), and each $t_i$ is a 128-bit vector, which is constant in SEV and SEV-ES processors. Therefore, the ciphertext $c$ of a plaintext $m$ at system physical address $A$ is then calculated by $c = E_K(m \oplus T(A))$.

\bheading{TLB structure.}
Although not explicitly documented, we conjecture SEV further extends TLB entries with two additional C-bits: gC-bit and nC-bit. The reason is that when address translation bypasses the page table walk, the values of the gC-bit and nC-bit are still required for the processor to determine which ASID to present to AMD-SP, if memory encryption is needed (see \tabref{tab:keyused}). Because the chosen ASID is different when ``gC-bit = 0 and nC-bit = 1'' and ``gC-bit = 1 and nC-bit = 0'', it is clear a single C-bit is not enough.

\yz{need justification}

\bheading{cache structure.}
Moreover, when loading a cache line, the C-bit from the page table entry or the TLB entry is copied into the cache tag to indicate it is encrypted data. While we could not find an explicit description of the cache tag structure from AMD's official documents, we conjecture a single C-bit (gC-bit $\oplus$ nC-bit) is also added into the cache tag. This is because when flushing out this cache line, the processor only needs this C-bit to determine if encryption is needed or not~\cite{kaplan:2016:sevWpaper}.

\yz{need justification}

==> disclosure.tex <==
1. In variant 2&3, why use 2 different VMs instead of directly using victim's VMCB?

Answer: use attack's VMCB will not obstruct victim's normal execution.

2. The percentage of decryption is misleading.

3. The variant 3 is not an attack.

4. 5.1.2 How to determine the rip/offset in SEV-ES?

5. 5.2 Crossline V1 on SEV-SNP. The RMP check during VMRUN will pass. But the remap is no longer possible.

6. The last paragraph in section 7 needs to rewrite.


TLBreach: 
The attack assumption.

The code for TLB flush will be moved to hardware and each vCPU will have a unique and dynamic tag. The tag management will look like ASID management but within hardware. This information will be stored in VMSA.
